The Dark Side of Perceptual Manipulations in Virtual Reality

"Virtual-Physical Perceptual Manipulations" (VPPMs) such as redirected walking and haptics expand the user's capacity to interact with Virtual Reality (VR) beyond what would ordinarily physically be possible. VPPMs leverage knowledge of the limits of human perception to effect changes in the user's physical movements, becoming able to (perceptibly and imperceptibly) nudge their physical actions to enhance interactivity in VR. We explore the risks posed by the malicious use of VPPMs. First, we define, conceptualize and demonstrate the existence of VPPMs. Next, using speculative design workshops, we explore and characterize the threats/risks posed, proposing mitigations and preventative recommendations against the malicious use of VPPMs. Finally, we implement two sample applications to demonstrate how existing VPPMs could be trivially subverted to create the potential for physical harm. This paper aims to raise awareness that the current way we apply and publish VPPMs can lead to malicious exploits of our perceptual vulnerabilities.

==> tex/VPPM.tex <==
\section{Defining Virtual-Physical Perceptual Manipulations (VPPMs)}\label{sec:vppms}

% define VPPMs 
\emph{Virtual-Physical Perceptual Manipulation} (\VPPM) refers to Extended Reality (XR) driven exploits that \textbf{alter the human multi-sensory perception of our physical actions and reactions to nudge the user's physical movements}
\footnote{We consider this definition to be one of the outcomes of this paper. It was derived from insights from our workshop and  discussions among all the authors. We present this definition early on in our paper (rather than in the results section) to make it easier for the reader to follow.}
(e.g.,  the position of body and hands). For example, redirected walking leverages visual dominance to change the VR user's walking direction and keep the user walking in a physical space. A {\VPPM} technique may vary in terms of prior consent and knowledge, and may also impact the user's ability to discern whether they are being manipulated. The user may be subjected to manipulation \textbf{knowingly or unknowingly} and the manipulation \textbf{may or may not be perceptible to the user}. Even if a user consents to being manipulated by {\VPPM}s, they might not be aware of the consequences of their physical actions. Crucially, regardless of consent or knowledge, \textbf{the intent behind a {\VPPM} is open to abuse} (e.g., disguising an attack as legitimate redirected walking) and may be opaque or disguised to the user. This ambiguity, in terms of consent to, awareness of, knowledge of, and intent behind a given {\VPPM} is what gives rise to the significant potential for harm.

% mention what we are looking at and what is out of scope and why
In this paper, we focus on what is arguably the worst-case scenario --- imperceptible {\VPPM}s are applied to the user unknowingly, without consent. 
In particular, we focus on the potential for harm at an individual level, where one VR user's physical actions (i.e., body motions) are manipulated to a physically abusive end. We defined this physically abusive outcome as physical harm --- an action that causes hurt or damage relating to the VR user's body.
The user is perceptually manipulated into a physical action, and they perceive their agency while performing physical actions. Note that we focus on \textit{perceptual manipulation} as opposed to \textit{physical manipulation}. This means that approaches that physically manipulate the user through external devices such as Electrical Muscle Stimulation (EMS) \cite{lopes_impacto_2015} and exoskeletons, are out of the scope of this paper. We exclude physical manipulations because in these cases, the VR user has had to wear/put on additional hardware, which suggests they are aware that these manipulations are elicited by the system.
Based on this definition, we explore what potential physical harm could be provoked to the VR user by manipulating their physical actions through {\VPPM}s, and how malicious actors could potentially abuse {\VPPM}s to provoke physical harm.







% Consequently, this assumption rules out approaches that physically manipulate the user into an action. For instance techniques and systems like electrical muscle stimulation \cite{lopes_impacto_2015} and exoskeletons.


% 1) knowingly/unknowingly (consent is a part of here) + perceptible/imperceptible
% 2) intent is unclear, lack attention and knowledge to address malicious attack.


%%%%%%%%%%%%%%%%%%% unused below
% Our target is a single VR user, manipulating physical actions (i.e., body motions) and physical harm. 




% and consider the potential physical harm to the user.
% focus on worst case: unknown user, imperceptible technique, one VR user, physical harm only
%We find a potential (imperceptible, nonconsensual + embodied motions) that VR manipulation could be used to enforce VR users to do certain actions.
% Crucially, the intent behind a VPPM may or may not be disclosed to the user, or the user may be deceived as to the intent.

% * i think the "steer or direct the user to a different physical end point or outcome" might need to be redrafted slightly to emphasize we are manipulating their physical movements (e.g. position of body, limbs etc) as physical end point might be a bit ambiguous or hard to understand on second reading
% * the imperceptible VPPMs are applied to VR users unknowingly + and whose intent are unknown to the user? The intent bit is the most tricky really, as in all classes they could still be used for an evil intent as opposed to an immersive/beneficial intent. Maybe we can simplify it to say as per the consent discussion that a VPPM may vary in terms of prior consent and knowledge, which may impact the user's ability to discern if they are being manipulated - but regardless of consent or knowledge, the intent behind a manipulation is open to abuse (e.g. disguising an attack as legitimate redirected walking) and may be opaque or disguised to the user

% % (e.g., electrical stimulation \cite{lopes_impacto_2015, lopes_providing_2017, aoyama_gvs_2017, auda_around_2019}, pressure \cite{kon_hanger_2018}, and force \cite{cheng_haptic_2014, ye_pull-ups_2019})
% Directly using external stimuli or forces can achieve the goal of manipulating a user's body motions. These approaches have been largely used to exploited kinesthetic haptic feedback. For example, when a VR user is flying upwards during a paragliding VR game, they can be lifted by human turkers (\textit{Haptic turk} \cite{cheng_haptic_2014}) or an active suspension system \cite{ye_pull-ups_2019}. Previous work also induced stimuli to trigger reflex actions to control VR user's body motions. For instance, \textit{electrical muscle stimulation} controls muscle contraction of VR user in order to generate impact feedback \cite{lopes_impacto_2015} or counter force while pushing heavy objects \cite{lopes_providing_2017}. \textit{Galvanic vestibular stimulation} elicits virtual acceleration by placing electrodes on the bilateral mastoids \cite{aoyama_gvs_2017}, and \textit{hanger reflex} exploits pressure on the user's head to create involuntarily rotations in VR \cite{kon_hanger_2018}. Besides kinesthetic haptics, Auda et al. \cite{auda_around_2019} used electrical muscle stimulation to manipulate VR user's walking direction in a limited physical space.
% % Unlike human turkers and active haptic system, activating user's reflex actions only requires wearable devices so that it is easier to deploy.

% These techniques are involuntary---VR users have no choice but carry out motions triggered by external stimuli. In these scenarios, users have a clear understanding of loosing their \textit{sense of agency}
% \cite{haggard_voluntary_2002, haggard_sense_2017, mueller_next_2020}, i.e., they know the motions are controlled by techniques instead of their own actions. In this work, we mainly focus on manipulations using narratives and perceptual illusions. Because they can be intrinsically embedded inside VR applications through software and interaction design, imperceptibly manipulating VR users to motions they unintended to do, or even harmful consequences.

==> tex/unused.tex <==
Virtual reality, as film, radio, and television, is also considered as a medium that allows for telling story through its virtual content \cite{pausch_disneys_1996}. Weech and colleagues \cite{weech_narrative_2020} showed enriched narratives was associated with increased presence. 

Perhaps the most direct example of manipulating user's body postures or motions comes to VR rhythm games \cite{llc_soundboxing_2016, fitterer_audioshield_2016, studio_beat_2019, lab_ohshape_2020}. For example, BeatSaber \cite{studio_beat_2019} player has to swing their arms to cut certain notes in different directions and avoid incoming walls by stepping away or squatting down. In OhShape \cite{lab_ohshape_2020}, players have to maintain different poses by putting their head and hands in the right spot, which can be dabbing, lunges, squats, or even choreography. Through these gaming design, VR rhythm game can make user do dancing poses originating from the song \cite{vr_fitness_insider_beat_2018}. On the other hand, research has leveraged virtual contents embedded in applications to control VR user's position in one-dimensional \cite{kastanis_reinforcement_2012}, two-dimensional displacement \cite{rovira_reinforcement_2017}, or hosting multiple VR users in a physical space \cite{marwecki_virtualspace_2018}. Current applications have already ``remote controlled'' player's actions but only within the safety boundary.


% \textit{device-gap}\footnote{The device-gap indicates that users have to put on display because of the form of current VR technology (HMD) so users have a clear gap between the reality and virtual experience. We argue there is also a device-gap in manipulating VR user's body motions, that is, whether VR users know themselves are being controlled.}


RW old
% current saftey boundary is not enough and VR fails happened
VR applications usually require an empty space as a safety boundary (e.g., Guardian system in Oculus) for users to perform interactions. However, having this safety space for VR interaction is not always the case in people's daily use. Conflicts between the virtual and physical environment can happen while users carry out some actions in VR but they are not aware of the consequences in the real world. This phenomenon, often referred to as VR fail, is recently starting to be explored in HCI. Dao et al. \cite{dao_bad_2021} presented a first classification of types and causes of VR fails by analysing YouTube videos. Their main focus was on a first categorization of accidents that are currently happening with consumer VR devices, while our work aims to explore if and how we can design applications through narratives and VR illusions to deliberately enforce VR fails.




Old introduction

% VR illusions are 
% The reason that VR illusion is Why the user acts accordingly in VR? In fact, combining all the information provided in a VR experience, the user perceives a sensory illusion while all the sensory input matches... (sensorimotor contigency?) three explanations of illusion in vr...

% mar's illusion model paper
%When these sensor-coupled stimuli match the brain’s expectations of what the next moment will bring, then the brain will tend to treat the simulated reality as real, which in turn will engage additional neural mechanisms to further the veracity of the illusion. 



% 1. VR illusion has been largely used in HCI and VR
% Virtual Reality (VR) has become increasingly popular, and current VR Head-Mounted Displays (HMDs) are getting more and more distributed among the general population \cite{yadav_why_2021}. VR has gained attention in the research community as well \cite{cipresso_past_2018}. In the field of Human-Computer Interaction (HCI), recent VR research has started leveraging human’s perceptual abilities to induce \emph{\PerceptualMani} --- an imperceptible manipulation on the user’s body motions --- that dominantly aims for positive purposes. For example, providing haptic feedback \cite{kohli_redirected_2010, azmandian_haptic_2016, cheng_sparse_2017}, redirected walking \cite{razzaque_redirected_2001, steinicke_estimation_2010}, weight perception \cite{rietzler_breaking_2018, samad_pseudo-haptic_2019}, and enhancing VR experience (e.g., ergonomic \cite{montano_murillo_erg-o_2017}, body posture \cite{shin_body_2020}).


% 2. (the critic of positive trend) the manipulative nature of illusion could be dangerous. Yet we have a lack of understanding on how to manipulate a user into damage though VR illusions
% The trend in HCI and VR is often times built upon the techno-positive framing where innovative ideas and designs tend to deliver the positive values. However, this paradigm often fails to consider its potential for malicious design \cite{greenberg_dark_2014, soden_chi4evil_2019, gugenheimer_exploring_2020}. The knowledge of \PerceptualMani\ also has a dark side and may be easily exploited to the detriment of the VR user. The field of VR and HCI currently has a lack of understanding to what degree an application could abuse or misuse a \PerceptualMani\ to result in potential harm to the user.

% 3. (what is this paper): why physical harm and vr illusion?; (how we do approach): through a design workshop, we explore what scenarios (what, damage) and how the participants use it to induce damage (how, technique).
% In this paper, our goal is to explore --- the dark side --- of {\PerceptualMani s} from the perspective of interaction design. To avoid being overly broad, we focus on the physical harm, an action that might cause hurt or damage relating to the VR user's body, spectators, or objects. We aim to investigate the following research questions (RQs):

% \begin{itemize}
%     \item RQ1: What could be the potential physical harm of \PerceptualMani?
%     \item RQ2: How to create the physical harm using \PerceptualMani\ through the perspective of dark (malicious) design?
%     \item RQ3: How can we prevent the dark side of \PerceptualMani?
% \end{itemize}

% % 4. (what we found) Results: harm dimensions, technique dimensions, types of harm/damage: illustrative examples + two (or three) demo examples to show how we can implement them.
% Current VR technologies are still unready for studying such future risks of \PerceptualMani. To overcome this problem, our method is conducting a focus-group \cite{morgan_focus_1996, krueger_focus_2015} speculative design workshop with designers and VR researchers (N=8). In the workshop we asked participants to speculate on scenarios where one could use {\PerceptualMani s} to manipulate the user’s body to induce what type of harm and how it could be done (RQ1 and RQ2). Through thematic analysis \cite{braun_using_2006}, we identified the space of physical harm, a 2 $\times$ 2 matrix with two variables --- the role of VR user (receiving or inducing) and the type of opponent (organism or object). Besides, we also present the types of how to abuse \PerceptualMani, including redirection techniques, the false-positive (what you see in VR is not in the real world), the false-negative (there are objects in the real world but not present in VR, e.g., system hazard, falling, colliding), and swapping (the VR content has a corresponding proxy but they are totally different: safari, Annexing realty, substitutional reality). These design spaces can help us to understand and create the application of abused/misused \PerceptualMani. Additionally, we articulated scenarios designed by our participants and implemented two [TWO/THREE DEMO EXAMPLES (SteppingOn, HittingFace)] to show how current interaction techniques in VR and HCI research could be potentially abused by malicious actors (RQ2).

% % 5. Finally, discuss through the lens of safety and security / ethics of VR research. What we can do for a next step?
% (RQ3) The main goal of this work is to demonstrate how {\PerceptualMani s} that are currently presented within the field of VR and HCI could potentially be abused by malicious forces. We also attempt to raise a discussion on two aspects. First, to start an exploration of the different types of potential harm that could be resulting from the use of VR illusions. Second, to discuss how we have to improve our current safety mechanisms to avoid these types of abusive designs.

% % 6. contributions
% This paper contains three contributions: 1) Through a thematic analysis, we identified a space of physical harm or damage through abusing VR illusion and the types of techniques showing how to do it from the results of design workshop; 2) illustrations of scenarios and two/three demo examples; and 3) we present reflections around the security and ethics of VR illusions.


% %Take Home
% Overall, we argue that VRManipulation techniques do have the potential to be misused to induce physical harm in the future and HCI as an academic discipline should become more captious publishing such work and also reflect on the potential for abuse. 
